AutoReP: Automatic ReLU Replacement for Fast Private Network Inference

The growth of the Machine-Learning-As-A-Service (MLaaS) market has highlighted clients' data privacy and security issues. Private inference (PI) techniques using cryptographic primitives offer a solution but often have high computation and communication costs, particularly with non-linear operators like ReLU. Many attempts to reduce ReLU operations exist, but they may need heuristic threshold selection or cause substantial accuracy loss. This work introduces AutoReP, a gradient-based approach to lessen non-linear operators and alleviate these issues. It automates the selection of ReLU and polynomial functions to speed up PI applications and introduces distribution-aware polynomial approximation (DaPa) to maintain model expressivity while accurately approximating ReLUs. Our experimental results demonstrate significant accuracy improvements of 6.12% (94.31%, 12.9K ReLU budget, CIFAR-10), 8.39% (74.92%, 12.9K ReLU budget, CIFAR-100), and 9.45% (63.69%, 55K ReLU budget, Tiny-ImageNet) over current state-of-the-art methods, e.g., SNL. Morever, AutoReP is applied to EfficientNet-B2 on ImageNet dataset, and achieved 75.55% accuracy with 176.1 times ReLU budget reduction.

==> Sections/Sec_related_works.tex <==
\section{Related works}
Secure MPC, a cryptographic technique, is used to allow multiple parties to jointly and securely perform a function while keeping each party's inputs private. MPC is capable of providing security guarantees as robust as those achievable by trusted third parties~\cite{canetti2001universally}. 
% For instance, with absolutely no information is leaked other than that can be obtained from the expected function outputs.
% Researchers have been using MPC to build secure, privacy-preserving DNN frameworks.
% \textcolor{blue}{Drawback of MPC} \\
% Although secure MPC for PPML and PI has smaller encryption overhead compared to HE based method \cite{lee2022privacy, huang2022cheetah}, it still comes with a order of magnitude higher computation \& communication overhead during encrypted evaluation compared to plaintext evaluation. The encryption overhead introduced by secure MPC protocol could potentially prohibit the popularity and the adoption of PPML in MLaaS application, especially for edge platforms such as mobile or IoT with limited resources. Thus, designing a scalable and provably secure DNN framework is considerably challenging, especially given that the current DNN model gets bigger and more complex. 
% \textcolor{blue}{Bottleneck of MPC} \\
% To reduce the latency and memory footprint overhead of secure MPC based PPML, we firstly need to identify the design bottleneck of MPC protocol in DNN inference. 
The DNN operators can be classified into 2 categories: linear operators and non-linear operators. Linear operator includes fully connected (FC) layer, convolutional layer and average pooling operator. Linear operator is evaluated based on encrypted multiplication using random Beaver triples \cite{beaver1991efficient} and addition, and it has a fair cost in secure MPC based PI. However, the non-linear operators, such as ReLU and sigmoid, requires garbled circuit \cite{knott2021crypten} based secure comparison protocol implementation, and the protocol normally leads to several order of magnitude higher computation and communication cost compared to plaintext counterpart. Unlike the plaintext evaluation where non-linear operator contribute to much smaller portion of latency compared to linear operator, the MPC based encrypted evaluation of non-linear operator leads to enormous latency overhead and becomes the major bottlenecks for PI application. 

% \subsubsection{Overhead Reduction of MPC Comparison Protocol.}
\subsection{Comparison Overhead Reduction Algorithms.}

% \textcolor{blue}{benefit and drawback of polynomial approximation} \\
% Existing MPC comparison protocol overhead reduction fall into three categories: \textit{ReLU (comparison) overhead reduction} by using model compression \cite{sanyal2018tapas, riazi2019xonn},  neural architecture search (NAS) for DNN model with smaller number of ReLUs \cite{aggarwal2020soteria, ghodsi2020cryptonas}, and fine-grained ReLU replacement with polynomial function \& ReLU dropping \cite{mishra2020delphi, ali2020polynomial, lou2020safenet, jha2021deepreduce}. 

TAPAS \cite{sanyal2018tapas} and XONN \cite{riazi2019xonn} compressed the model into binary neural network format which has reduced number of bits, and the method can effectively reduce the size of Garbled circuit for MPC comparison protocol implementation. CryptoNAS \cite{ghodsi2020cryptonas} and Sphynx \cite{cho2021sphynx} are two typical NAS directed works which define searched spaces with reduced count of ReLU and MaxPool and find the suitable architecture. Delphi\cite{mishra2020delphi}, SafeNet \cite{lou2020safenet}, and Cho's work~\cite{cho2022selective} focus on partially replacing ReLU function with polynomial function to achieve speedup in MPC based PI.  
However, polynomial replacement of ReLU often comes with a non-negligible model accuracy degradation. The reduction of non-polynomial operators (e.g., ReLU or maxpool) in these works still leads to a severe accuracy drop due to their frameworks' limitation, and they can not achieve comparison free PI implementation. To maintain accuracy, a low ReLU reduction ratio needs to be used. As a result, these works suffer from high latency due to limited computation and communication saving. Furthermore, none of the aforementioned methods have been validated in large scale model and dataset, such as ResNet 50 structure on ImageNet, which put a doubt on the scalability of those works. 

\subsection{Hardware Acceleration of Secure DNNs.}
% \textcolor{blue}{hardware acceleration approaches} \\
% The energy efficiency challenge \textcolor{red}{???} of secure DNN models motivates the second trend: {\em hardware acceleration}. 
The growing computing capability and energy efficiency of computing platforms such as CPUs, GPUs and FPGAs mitivates the second trend: {\em hardware acceleration for PI}. 
The state-of-the-art secure DNNs using MPC are mainly implemented on CPUs. For instance, CrypTFlow~\cite{kumar2020cryptflow} converts TensorFlow inference code~\cite{abadi2016tensorflow} into MPC protocols at the push of a button using Intel SGX. MP-SPDZ~\cite{keller2020mp} primarily targets at the compiler level, i.e., compile the high-level secure protocol code (bytecode) into virtual machine. CrypTFlow2~\cite{rathee2020cryptflow2} further improves CrypTFlow by using Athos, an end-to-end compiler, to convert TensorFlow to MPC protocols.
% It uses a 3.7 GHz Intel Xeon processor (CPU) consisting of 4 cores and 16 GBs of RAM.  
GAZELLE~\cite{juvekar2018gazelle} uses a combination of homomorphic encryption (HE) and traditional two-party computation techniques (such as garbled circuits) on Intel Xeon E5-2666 CPU with 7.5GB memory and demonstrates three orders of magnitude faster inference time, compared with fully homomorphic approaches such as CryptoNets~\cite{gilad2016cryptonets}. 
%Prior arts mainly focus on CPU (e.g., CrypTFlow~\cite{kumar2020cryptflow}, MP-SPDZ~\cite{keller2020mp}, GAZELLE~\cite{juvekar2018gazelle}) and GPU (e.g., CryptGPU~\cite{tan2021cryptgpu}) implementations. 

Recently, a DNN system built on graphics processing unit ({GPU}) using MPC, titled CryptGPU~\cite{tan2021cryptgpu}, has been discussed. 
%has drawn attention from both academia and industry. 
CryptGPU embeds cryptographic operations over secret-shared values into the floating-point operations for CUDA kernels. It achieves up to 150$\times$ speedups over CPU-based solutions. Later, CryptGPU work is incorporate into Crypten framework~\cite{knott2021crypten} to enable easy to use pytorch-based MPC framework with GPU acceleration backend. 

\subsection{Activation Pruning.}

